On the Lie bracket approximation approach to distributed optimization: Extensions and limitations

We consider the problem of solving a smooth convex optimization problem with equality and inequality constraints in a distributed fashion. Assuming that we have a group of agents available capable of communicating over a communication network described by a time-invariant directed graph, we derive distributed continuous-time agent dynamics that ensure convergence to a neighborhood of the optimal solution of the optimization problem. Following the ideas introduced in our previous work, we combine saddle-point dynamics with Lie bracket approximation techniques. While the methodology was previously limited to linear constraints and objective functions given by a sum of strictly convex separable functions, we extend these result here and show that it applies to a very general class of optimization problems under mild assumptions on the communication topology.

==> myStandardPreamble_arXiv.tex <==
% change @-symbol interpretation for using macros
\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% =============================
% ===         M I S C      ====
% =============================

% extended TeX
\@ifpackageloaded{etex}{}{\RequirePackage{etex}}

% keeps relative paths when including different .tex-files
% use \subimport*{subdirectory}{tex-File} to input tex-Files
\@ifpackageloaded{import}{}{\usepackage{import}}

% nice tables
\@ifpackageloaded{booktabs}{}{\usepackage{booktabs}}

% microtype for better spacing of letters
%\@ifpackageloaded{microtype}{}{\usepackage{microtype}}

% calculations also in tex-Code
\@ifpackageloaded{calc}{}{\usepackage{calc}}

% if conditions
\@ifpackageloaded{ifthen}{}{\usepackage{ifthen}}


% =============================
% ===    G R A P H I C S    ===
% =============================
\@ifpackageloaded{graphicx}{}{\usepackage{graphicx}}
\@ifpackageloaded{xcolor}{}{\usepackage{xcolor}}


% =============================
% ===         T I K Z      ====
% =============================
\@ifpackageloaded{tikz}{
     \usetikzlibrary{arrows,shapes,patterns,positioning,calc}
     }{
     \usepackage{tikz}
     \usetikzlibrary{arrows,shapes,patterns,positioning,calc}
}
\@ifpackageloaded{pgfplots}{
     }{
     \usepackage{pgfplots}
     }
% SOME TIKZ STYLE DEFINITIONS
\tikzstyle{boxstyle}=[draw=black,inner sep=7pt]      % style for boxes in blockdiagrams
\tikzstyle{arrowstyle}=[]                            % style for arrows in blockdiagrams



% =============================
% ===         M A T H      ====
% =============================
\@ifpackageloaded{amsmath}{}{\usepackage{amsmath}}
\@ifpackageloaded{amsfonts}{}{\usepackage{amsfonts}}
\@ifpackageloaded{amssymb}{}{\usepackage{amssymb}}
\let\theoremstyle\relax
\@ifpackageloaded{amsthm}{}{\usepackage{amsthm}}
\@ifpackageloaded{yhmath}{}{\usepackage{yhmath}}
\@ifpackageloaded{mathdots}{}{\usepackage{mathdots}}


% =============================
% ===    H Y P E R R E F    ===
% =============================

% some color definitions
\colorlet{lcolor}{green!45!black}
\colorlet{ucolor}{magenta!40!black}
\colorlet{ccolor}{green!40!black}

% hyperref for internal links
\usepackage[colorlinks=true,%
            linkcolor=lcolor,%
            urlcolor=lcolor,%
            citecolor=lcolor]{hyperref}

% cleverref for automatically labeling of references
\usepackage[nameinlink,capitalise]{cleveref}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% rechange @-symbol interpretation
\makeatother

